On the Theory and Practice of Privacy-Preserving Bayesian Data Analysis

Bayesian inference has great promise for the privacy-preserving analysis of sensitive data, as posterior sampling automatically preserves differential privacy, an algorithmic notion of data privacy, under certain conditions (Dimitrakakis et al., 2014; Wang et al., 2015). While this one posterior sample (OPS) approach elegantly provides privacy "for free," it is data inefficient in the sense of asymptotic relative efficiency (ARE). We show that a simple alternative based on the Laplace mechanism, the workhorse of differential privacy, is as asymptotically efficient as non-private posterior inference, under general assumptions. This technique also has practical advantages including efficient use of the privacy budget for MCMC. We demonstrate the practicality of our approach on a time-series analysis of sensitive military records from the Afghanistan and Iraq wars disclosed by the Wikileaks organization.

==> relwork.tex <==
\section{Related Work}

The two main pieces of work that deal with Bayesian inference and differential privacy are~\cite{dimitrakakis2013} and~\cite{wang2015}. \cite{dimitrakakis2013} looks at some popular prior-posterior pairs used in Bayesian inference and characterizes the conditions under which directly sampling from these posteriors is differentially private; they also consider a variation of differential privacy where the effect of changing the private value of a single individual {\em{by a small amount}} is low. Motivated by the exponential mechanism, \cite{wang2015} introduces a generic differentially private mechanism for sampling from a posterior that obeys a certain sensitivity condition; they also provide a private MCMC procedure for sampling from such a posterior that is motivated by the Stochastic Gradient Langevin Dynamics (SGD-LD) method of~\cite{wt11}.

There has also been a great deal of work in differentially private frequentist methods, much of which relates to convex optimization. Differentially private non-convex optimization, including clustering, on the other hand, is considered more challenging. \cite{NRS07} provides an algorithm and an associated analysis for differentially private clustering of points in space, while~\cite{kddkmeans} provides algorithms along with an experimental evaluation. \cite{WWS15} provides two algorithms along with experiments for differentially private subspace clustering. To our knowledge, there is no previous work on differentially private clustering of time series data. 

